FloatGate: Contact-Risk-Aware Visual Updates for Free-Floating Capture in Simulated Spacecraft Cabins

A free-floating target can translate and tumble while a robot computes a grasp action. Updating more visual information can therefore improve perception while making the action less timely. We study this trade-off in simulated spacecraft cabins and introduce FloatGate, a contact-error-based visual budget selector. Offline candidate branches advance dynamics during budget-dependent computation and evaluate one committed action block. A lightweight head conditions on target, cache, and execution state to select one admissible budget before policy inference. The method reuses sparse encoding and caching; its contribution is the allocation objective. Across eight policy seeds and 10,240 paired episodes per method, FloatGate reaches 84.9% retention versus 76.1% for full event-assisted updates, while mean request time falls from 67.0 to 47.5 ms. A crossed supervision-clock study narrows the gain over execution-aligned action supervision to 0.89 points (95% interval -0.86 to 2.64). A separate matched-state audit examines action replacement, pre-consumption acquisition, and agreement with a local budget oracle. The point advantage over aligned action supervision and its interaction with the label clock remain statistically unresolved. These results concern fixed-base near-field capture with supplied CAD, not hardware or on-orbit capability.

==> main_external_labels.tex <==
% Generated cross-file references; external targets are deliberately not hyperlinked.
\makeatletter
\newlabel{sec:protocolsupp}{{A}{1}{}{}{}}
\newlabel{sec:clockprotocol}{{A.3}{1}{}{}{}}
\newlabel{sec:branchrollout}{{A.4}{2}{}{}{}}
\newlabel{sec:riskprotocol}{{A.5}{2}{}{}{}}
\newlabel{sec:analyticbaseline}{{A.6}{3}{}{}{}}
\newlabel{eq:alignedaction}{{S6}{4}{}{}{}}
\newlabel{sec:decisionaudit}{{A.7}{4}{}{}{}}
\newlabel{eq:shortwindow}{{S7}{5}{}{}{}}
\newlabel{eq:localoracle}{{S8}{5}{}{}{}}
\newlabel{sec:analysissupp}{{B}{7}{}{}{}}
\newlabel{tab:nativebaseline}{{S1}{7}{}{}{}}
\newlabel{tab:decisionquality}{{S2}{7}{}{}{}}
\newlabel{tab:delaycontrol}{{S3}{8}{}{}{}}
\newlabel{fig:delay}{{S1}{8}{}{}{}}
\newlabel{tab:labelcontrol}{{S4}{8}{}{}{}}
\newlabel{tab:onlinegate}{{S5}{9}{}{}{}}
\newlabel{tab:gateseed}{{S6}{9}{}{}{}}
\newlabel{tab:gatereasons}{{S7}{9}{}{}{}}
\newlabel{tab:nonideal}{{S8}{10}{}{}{}}
\newlabel{tab:robustness}{{S9}{10}{}{}{}}
\newlabel{fig:tracker}{{S2}{11}{}{}{}}
\newlabel{tab:tracker}{{S10}{11}{}{}{}}
\newlabel{tab:modalityfactorial}{{S11}{11}{}{}{}}
\newlabel{tab:ablation}{{S12}{11}{}{}{}}
\newlabel{fig:calibration}{{S3}{12}{}{}{}}
\newlabel{tab:calibration}{{S13}{12}{}{}{}}
\newlabel{fig:timing}{{S4}{13}{}{}{}}
\newlabel{tab:timingfull}{{S14}{13}{}{}{}}
\newlabel{tab:cost}{{S15}{13}{}{}{}}
\newlabel{sec:visualsupp}{{C}{14}{}{}{}}
\newlabel{fig:events}{{S5}{14}{}{}{}}
\newlabel{fig:videoevents}{{S6}{15}{}{}{}}
\newlabel{fig:selection}{{S7}{16}{}{}{}}
\newlabel{fig:risk}{{S8}{17}{}{}{}}
\newlabel{fig:failures}{{S9}{18}{}{}{}}
\makeatother

